Real-Time Gaze Tracking with Event-Driven Eye Segmentation

Gaze tracking is increasingly becoming an essential component in Augmented and Virtual Reality. Modern gaze tracking al gorithms are heavyweight; they operate at most 5 Hz on mobile processors despite that near-eye cameras comfortably operate at a r eal-time rate ($>$ 30 Hz). This paper presents a real-time eye tracking algorithm that, on average, operates at 30 Hz on a mobile processor, achieves \ang{0.1}--\ang{0.5} gaze accuracies, all the while requiring only 30K parameters, one to two orders of magn itude smaller than state-of-the-art eye tracking algorithms. The crux of our algorithm is an Auto~ROI mode, which continuously pr edicts the Regions of Interest (ROIs) of near-eye images and judiciously processes only the ROIs for gaze estimation. To that end, we introduce a novel, lightweight ROI prediction algorithm by emulating an event camera. We discuss how a software emulation of events enables accurate ROI prediction without requiring special hardware. The code of our paper is available at https://github.com/horizon-research/edgaze.

==> related.tex <==
\section{Related Work}
\label{sec:related}


% \paragraph{Gaze Estimation} By large, gaze estimation can be classified into two main categories, model-based methods and appearance-based methods. Appearance-based methods directly use the eye image as input and predict the gaze direction~\cite{zhang2015appearance, wood2016learning, lu2014adaptive}. On the other hand, model-based methods use a geometric eye model to predict gaze direction. Examples includes DeepVOG~\cite{yiu2019deepvog}, etracker~\cite{li2018etracker}. These methods use near eye camera and a pre-constructed geometric model to estimate gaze. Others use \fixme{unconventional} cameras, such as RGB-D camera~\cite{jianfeng2014eye} or event camera~\cite{angelopoulos2020event}. Although those studies can achieve high accuracy, general mobile devices are not accessible to those hardware. In our study, we choose to use conventional camera to demonstrate the applicability of our work.

\paragraph{Region Proposal} Many studies have proposed region proposal algorithms in different computer vision tasks to reduce the overall computation and data transmission~\cite{kong2016hypernet, ren2015faster, girshick2015fast, girshick2014rich, he2017mask, kodukula2021rhythmic, mudassar2019camera}. Prior works such as, fast R-CNN~\cite{girshick2015fast} and faster R-CNN~\cite{ren2015faster} proposed region proposal networks for general objects. Their region proposal networks rely on the initial feature extraction, which is not computationally lightweight. Others~\cite{kodukula2021rhythmic, mudassar2019camera}, passively react based on the previous result, they are not suitable for tasks, like eye tracking, which need to actively track fast movements. Our region proposal network is tailored for eye tracking, and it is inspired by event cameras and can effectively predict the quick eye movements between two frames. In addition, our network is lightweight and more suitable for mobile devices compared to prior region proposal networks~\cite{girshick2015fast, ren2015faster}.


\paragraph{In-Sensor Computing} The idea of in-sensor computing have been proposed by many prior works~\cite{??}. As camera sensors have been assigned more computational power, today's cameras are able to capture more appealing images. For instance, today's camera is capable of performing face detection in order to have a better auto-focusing~\cite{camera-auto}. Industries have also designed dedicated camera sensors, such as pixel visual core~\cite{redgrave2018pixel}, so that cameras are able to perform a wide range of tasks, such as white balancing, HDR, faster and more efficient~\cite{googlevisualcore}. Unlike previous camera designs, which focus on improving image visual quality, we leverage the in-sensor computing to accelerate visual applications, while being more energy-efficient. 




==> sensor.tex <==
\subsection{Reducing Sensor Data Transmission}
\label{sec:framework:sensor}

\fixme{I think you have another copy of this text in another .tex file}

So far we have focused on improving the compute efficiency the eye tracking algorithm. However, the data transmission overhead from the image sensor to the processor (that executes the eye tracking algorithm) is non-negligible. A recent characterization study from Facebook shows that the average energy consumption of data transmission, per byte, from the sensor to the processor chip (through the industry-standard MIPI CSI-2 interface~\cite{mipicsi2}) consumes about 800 times higher energy than the computation energy per byte~\cite{liu2019intelligent}. Similar observations are made in other recent studies~\cite{kodukula2021rhythmic, ??}.

The auto-ROI capability of our eye tracking algorithm inherently provides an opportunity to reduce the data transmission overhead. Our idea is to execute part of the algorithm inside the image sensor to reduce the data transmission \textit{volume} and thereby the transmission energy. In-sensor computing is possible as image sensor vendors have started integrating processing capabilities with the conventional pixel array in one sensor, sometimes in one single chip~\cite{chai2020sensor, kwon2020low, haruta20174}. A recent example is the IMX 500 image sensor from Sony that provides dedicated memories and a digital signal processor for executing DNNs~\cite{imx500}.

\begin{table}[ht]
\caption{Total number of Floating Point Operations (FLOPs) and the output data size of the four major components in our algorithm under a $640\times400$ grayscale input. As a ballpark estimate, we assume the ROI image is one-third the size of a full-resolution and half of the frames are extrapolated. We show the full-resolution image size for the reference. Recall that data transfer consumes 800 times more energy than computation per byte~\cite{liu2019intelligent}.}
\centering
\resizebox{1\columnwidth}{!}{
\renewcommand*{\arraystretch}{1}
\renewcommand*{\tabcolsep}{2pt}
\begin{tabular}{c c c c c | c}
\toprule[0.15em]
\textbf{Stages} & \textbf{\specialcell{~Event Map\\ Generation}} & \textbf{\specialcell{~Edge Map\\ Generation}} & \textbf{\specialcell{Prediction\\~Network}}  & \textbf{\specialcell{~~~~Seg.\\Network}} & \textbf{\specialcell{Full-res\\~Image}}\\
\midrule[0.05em]
\# of MAC (Million) & 0.3 & 1.9 & 55.4 & 2920.0 & NA \\ 
%\midrule[0.05em]
Output Data (KB) & 7.81 & 7.81 & 41.7 & 62.5 & 250 \\ 
\bottomrule[0.15em]
\end{tabular}
}
\label{table:pipeline_mac}
\end{table}
% event map and edge map are 1/2 size of orginal image
% event map size should be (320*200)/8
% edge map # Mac = (320*200)*(25+4+1)
% event map should be (320*200)*4

While conceptually simple, reaping the reward of in-sensor computing is not trivial. Computation inside image sensors consumes more energy than that on a backend processor. This is because the semiconductor fabrication technology, quantified by the \textit{process node}, of the sensor usually lags at least one generation behind that of the processor. Many (mobile) processes are fabricated using a 7~nm process node, but even high-end image sensors today still use a 14~nm or or 28~nm process node~\cite{??}. The computation power consumption increases quadratically with respect to the process node~\cite{dennard1974design}. Therefore, one must carefully weigh the reduction of data transmission energy against the overhead of computing inside an image sensor.

\begin{figure}[t]
    \centering
    \subfloat[No compute in sensor.]{
      \label{fig:mode1}
      \includegraphics[width=0.31\columnwidth]{mode1}
    }
    \hfill
    \subfloat[Predict ROI in sensor.]{
      \label{fig:mode2}
      \includegraphics[width=0.31\columnwidth]{mode2}
    }
    \hfill
    \subfloat[Optimal mapping.]{
      \label{fig:mode3}
      \includegraphics[width=0.31\columnwidth]{mode3}
    }
    \caption{Different mapping schemes from the four major algorithmic components, event map generation (EvMapGen), edge map generation (EdMapGen), ROI prediction network (PredNet), and eye segmentation network (SegNet), to hardware. The optimal mapping (c) minimizes the total data transmission and computation energy.}
    \label{fig:mapping}
\end{figure}

Our goal is thus to map the different components of our eye tracking algorithm to the sensor and processor in such a way that the total energy consumption is minimized. Intuitively, the ideal mapping is one where a trivial amount of computation in the sensor can drastically reduce the data communication.

To identify the optimal mapping, we first quantify the computation cost and the output data volume of the four main components in our algorithm: event map generation, edge map generation, prediction network, and segmentation network, the former three comprise the ROI prediction algorithm (\Fig{fig:bbox_prediction}). \Tbl{table:pipeline_mac} shows the results. Note that each image pixel takes 1 byte; each pixel in the event map and the edge map takes 1 bit; each segmentation map pixel takes 2 bits (4 classes).

The entirety of the ROI prediction algorithm (column 2--4 in \Tbl{table:pipeline_mac} combined) is much more lightweight than the segmentation network, requiring less than 2\% of Floating Point Operations (FLOPs) of the latter. One straightforward solution would thus be to map the entire ROI prediction algorithm to the sensor while leaving only the segmentation network in the processor chip. This mapping is shown in \Fig{fig:mode2}.

Compared to the mapping in today's system where all the computation takes place in the processor (illustrated in \Fig{fig:mode1}), predicting ROI in the sensor reduces the data transmission volume from the full-resolution image to only the ROI image (from sensor to processor) and the segmentation map (from the processor back to the sensor); the reduction in data transmission overhead will outweigh the slight computation energy increase of moving the ROI prediction to the sensor given the little computation of the ROI prediction algorithm.

Interestingly, mapping the ROI prediction network to the sensor is \textit{not} the most energy-efficient mapping. We propose a mapping, shown in \Fig{fig:mode3}, where only the event map generation and the prediction network execute in the sensor while the edge map generation and the segmentation execute on the processor. Compared to \Fig{fig:mode2}, our mapping reduces both the data transmission volume (since the edge map, rather than the segmentation map, is transmitted) and the computation energy (since the edge map is generated in the processor).

%Therefore, to deploy our framework for in-sensor computing, the mode-switching algorithm \circled{white}{3} in \Fig{fig:eye_tracking} can be deployed on camera sensors due to its own lightweight nature, and the rest of pipeline can be deployed on the backend processor. by doing so, some modes in \circled{white}{4} do not need to request the entire image frame from the camera sensor, we can reduce the average data transmission between the camera sensor and the backend processor. For instance, when executing the ``ROI-only segmentation'' mode, only the pixels within the ROI need to be transferred to the backend processor with some control signals. In the mode of ``ROI-based Extrapolation'', no pixel needs to be transferred, only the control signals need to be transferred to the backend processor. 




